Symbolic dynamics for the Kuramoto-Sivashinsky PDE on the line II

We prove the existence of infinite number of homoclinic and heteroclinic orbits to two periodic orbits for the Kuramoto-Sivashinsky PDE on the line with odd and periodic boundary conditions and for some fixed parameter value of the system. The proof is computer assisted and it is based on a new algorithm for rigorous integration of the variational equation for a class of dissipative PDEs on the torus.

==> c1conver.tex <==
\section{$\mathcal C^1$-convergence of Galerkin projections}
\label{sec:c1-conver}
 The goal of this section is to formulate results regarding the convergence of solutions to Galerkin projections and associated variational equations to the solution of underlying dissipative PDE. This, along with bounds obtained from the algorithm, will give us bounds on partial derivatives of solutions to PDE with respect to the initial conditions.


We will be dealing with $H \subset \mathbb{R}^{\mathbb{Z}_+}$, i.e. with sequences $(a_1,a_2,\dots)$,  with some norm $\|\cdot\|$. Let
$e_i$ denote the sequence such that $(e_i)_j=0$ for $j \neq i$ and $(e_i)_i=1$. By $e_j^* \in H^*$ we denote a dual form, $e^*_j(e_i)=\delta_{ij}$.
If $J \subset \mathbb{Z}_+$, then by $P_J$ we denote projection $\pi_i(P_J(w))=w_i e_i$ for $i \in J$ and $\pi_i(P_J(w))=0$ if $i \notin J$.

We assume that we have increasing family of finite subsets of $\mathcal{Z}_+$  $J_1  \subsetneq  J_2  \subsetneq J_n \dots  $, such that $\bigcup_{n \in \mathbb{Z}_+} J_n = \mathcal{Z}_+$.
For $n \in \mathbb{Z}_+$  by $H_n$ we will denote a subspace spanned by
$\{e_j\}_{j \in J_n}$ by $P_n$ we denote the projection on $H_n$ and let $Q_n=\mathrm{Id}-P_n$.

 Let $\pi_k$ be a projection onto $k$-th direction, i.e. $\pi_k(\sum w_j e_j)=w_ke_k$.


We will assume that $H \subset \mathbb{R}^{\mathbb{Z}_+}$  with a norm $\|\cdot\|$ be a Banach space, which is \gss space (see \cite{WZ24}  \textbf{PZ: dac cos z tego tutaj lub w appendixie}).

We investigate the Galerkin projections of the following problem
\begin{equation}
  u'=F(u)=L(u) + N(u), \label{eq:feqLN}
\end{equation}
where $L$ is a linear operator and $N$ is a nonlinear part of F. They are given by
\begin{equation}\label{eq:GalerkinODE}
u'=P_n(F(u)),\qquad u(0)=P_nu_0.
\end{equation}
Denote by $\varphi^n$ a local dynamical system on $H_n$ induced by
the $n$-th Galerkin projection.

We need to introduce  the notation for Galerkin projections of our vector field.  Let $\iota_n: H_n \to H$ be the imbedding of $H_n$ into
$H$. Then we define $F^n:H_n \to  H_n$ by $F^n(z)=P_n (F(\iota_n(z))$, i.e. this is simply a Galerkin projection.


%We assume that the basis $e_1, e_2, \dots$ of $H$ is built from
%eigenvectors of $L$. We assume that the corresponding eigenvalues
%$\lambda_k$ (i.e. $Le_k=\lambda_k e_k$) are ordered so that
%\begin{displaymath}
%  \lambda_1 \geq \lambda_2 \geq \dots, \quad \mbox{and} \quad \lim_{k\to \infty} \lambda_k=-\infty.
%\end{displaymath}
%Hence $L$ can  have only a finite number of positive eigenvalues.


We assume that $F_i$ is a formal power series in variables $a_k$ and symbols $\frac{\partial^k F_i}{\partial a_{i_1} \dots \partial a_{i_k}}$ are defined by formal
differentiation of $F_i$.

\begin{definition}
\label{def:Fadmisible}
  We say that $F$ is admissible, if $P_nF $ is defined on $H_n$ and is $\mathcal{C}^3$ as a function defined on $H_n$.
\end{definition}

\begin{definition}
\label{def:C1C2C3}
Assume that $(H,\|\cdot\|)$ is \gss space.
Let  $W\subset H$ and $F:\mathrm{dom}(F) \to H$.  Assume that $F$ is admissible. We say that
$F$ satisfies conditions {\rm \textbf{C1}}, {\rm \textbf{C2}}, {\rm \textbf{C3}}, {\rm \textbf{C4}} on $W$ if
\begin{description}
\item[C1] There exists $M \geq 1$, such that $P_n(W) \subset W$
for $n \geq M$
\item[C2] $W$ is compact.
\item[C3]  $W \subset \dom(F)$, ( for each $u \in W$ $F(u) \in H$) and  function   $F:W \to H$ is continuous.
\item[C4]  for every $i$ and $z \in W$  there exists $\lim_{n \to \infty} D(F_{i|H_n }) (P_n z)$ and we define
\begin{equation*}
  \widetilde{D F}_i(z)= \lim_{n \to \infty} D(F_{i|H_n }) (P_n z).
\end{equation*}
We assume that $ \widetilde{D F}_i: W \to H^*$ is continuous.

\end{description}
\end{definition}
Observe that conditions C1, C2, C3, C4  (called later \emph{convergence conditions}) have nothing to do with splitting $F=L+N$ and $e_i$ being eigenvectors of $L$.

Conditions C1, C2, C3 are needed for convergence of Galerkin projections ($C^0$-convergence), while C4   is  required (plus some other conditions) for convergence of solutions of variational equations for Galerkin projections ($C^1$-convergence).


Let us comment on condition \textbf{C4}.  Instead of introducing $\widetilde{DF}_i$ one can be tempted to replace it by \newline
for every $i$   $W \subset \dom\left(DF_i\right)$ and function $DF_i:W \to H^*$ is continuous. \newline
This approach  is problematic, because it may happen that $F_i$ is not defined everywhere and the notation of Frechet derivative cannot be applied.

However, using $\widetilde{DF}_i$ we will have the following formula  (if $W$ is convex)
\begin{equation*}
F_i(z) - F_i(w)= \int_0^1 \widetilde{DF}_i(t z + (1-t)w)dt \cdot (z - w),  \quad z,w \in W. % \label{eq:dFi-int}
\end{equation*}
This result  is obtained in   \cite{WZ24}  \textbf{PZ: dac lepsze wspolrzedne}.




\begin{definition}
\label{def:Dlog}
We say that $F$ satisfies condition {\rm \textbf{D}},
 on $W \subset H$ if $W$ is convex and  \\
 there exists  $l \in \mathbb{R}$ such that for all
$n=1,2,\dots$
\begin{equation*}
   \sup_{x \in P_n W}\mu\left(D P_n F_{|H_n} (x) \right) \leq l.
\end{equation*}
\end{definition}
The main idea behind  condition \textbf{D} is to ensure that the
logarithmic norms (see Appendix~\ref{sec:lognorm}) for all Galerkin projections are uniformly
bounded.



The following theorem is a generalization of \cite{Z} (Thm. 13). There   it is assumed that  $W$ is a trapping region and  $H=l_2$ was used, but  the main idea  proof is the same.  The proof is given in \cite{WZ24}  \textbf{dac  lepsze wspolrzedne}.
\begin{theorem}
\label{thm:limitLN}
 Assume $(H,\|\cdot\|)$ is \gss.
   Assume that $W \subset H$ and $F$ satisfy conditions {\rm \textbf{C1}}, {\rm \textbf{C2}}, {\rm \textbf{C3}}, {\rm \textbf{D}} and $W$ is convex. Let $Z\subset W$ and $T>0$ be such that all $n>M_1$ there holds
  \begin{equation*}
    \varphi^n(t,x)\in W\quad \text{for } x\in P_n(Z), t\in[0,T]
  \end{equation*}
    Then
    \begin{description}
    \item[1.]{\bf Uniform convergence and existence} For a fixed $u_0 \in Z$,
    let  $u_n:[0,T] \to P_n(W)$ be a solution of (\ref{eq:GalerkinODE}).
    Then $u_n$ converges uniformly to a function
     $u^*:[0,T]\to W$, which is a solution of (\ref{eq:feqLN}) and $u^*(0)=u_0$. The
    convergence of $u_n$ is uniform with respect to $u_0 \in Z$.
    \item[2.] {\bf Uniqueness within $W$}. There exists only one solution of the initial
     value problem (\ref{eq:feqLN}), $u(0)=u_0$ for any $u_0 \in Z$, such that $u(t) \in W$
     for $t\in[0,T]$.
    \item[3.]  {\bf Lipschitz constant}. Let $u:[0,T] \to W$ and
      $v:[0,T] \to W$ be solutions of (\ref{eq:feqLN}) with $u(0),v(0)\in Z$. Then
      \begin{equation}
         |v(t) - u(t) | \leq e^{lt}|v(0) - u(0)|\quad \text{for } t\in[0,T]. \label{eq:LipConstant}
      \end{equation}
    \item[4.] {\bf Semidynamical system.} The partial map $\varphi:[0,T] \times W \to W$, where
       $\varphi(\cdot,u_0)$ is a unique solution of equation (\ref{eq:feqLN}), such that
       $\varphi(0,u_0)=u_0$ defines a semidynamical system on $W$, namely
        \begin{itemize}
          \item $\varphi$ is continuous
          \item $\varphi(0,u)=u$
          \item $\varphi(t,\varphi(s,u)) = \varphi(t+s,u)$
        \end{itemize}
    provided $\varphi(t+s,u)$ exists.
  \end{description}
\end{theorem}
Observe that the essential difficulty in application of the above theorem is to find set $W$. A systematic way to construct it is based on  the \emph{isolation property}, which is related
to splitting  $F=L+N$ and the diagonal form of $L$.

\subsection{Isolation property}

To illustrate the \emph{isolation property}
let us consider a class of dissipative PDEs of the following form
\begin{equation}
  u_t = L u + N\left(u,Du,\dots,D^ru\right), \label{eq:genpde}
\end{equation}
where $u \in \mathbb{R}^n$,  $x \in \mathbb{T}^d=\left(\mathbb{R}\mod 2\pi\right)^d$, $L$ is a linear operator, $N$ is a
polynomial and by $D^s u$ we denote $s^{\text{th}}$ order derivative of
$u$, i.e. the collection of all spatial partial derivatives of $u$ of
order $s$. The reason to consider polynomial and not more general functions $N$ is technical --- we need to compute
the Fourier coefficients of $N\left(u,Du,\dots,D^ru\right)$. This can be achieved by taking suitable convolutions of Fourier expansions of $u$ and its spatial partial derivatives.

We require, that the operator $L$ is diagonal in the Fourier basis
$\{e^{ikx}\}_{k \in \mathbb{Z}^d}$,
\begin{equation*}
  L e^{ikx}= -\lambda_k e^{ikx},
\end{equation*}
with
\begin{eqnarray*}
 L_* |k|^p &\leq& \lambda_k \leq  L^* |k|^p, \qquad \text{for all $|k| > K$ and  $K,L_*,L^* \geq 0$}, \\
    p &>& r.
\end{eqnarray*}

If the solutions are sufficiently smooth, the problem (\ref{eq:genpde}) can be written as an infinite ladder of ordinary differential equations for the Fourier
coefficients in $u(t,x)=\sum_{k \in \mathbb{Z}^d} u_k(t) e^{i kx}$, as follows
\begin{equation}
  \frac{d u_k}{dt} = F_k(u)=-\lambda_k u_k + N_k\left(\{u_j\}_{j \in \mathbb{Z}^d}\right), \qquad \mbox{for all
  $k \in \mathbb{Z}^d$}. \label{eq:fueq}
\end{equation}



The crucial fact, which makes our approach to the rigorous integration of (\ref{eq:fueq})  possible is the \emph{isolation property}, which reads:

\emph{Let}
\begin{equation*}
   W=\left\{ \{u_k\}_{k \in \mathbb{Z}^d}\,|\,  |u_k| \leq \frac{C}{|k|^s q^{|k|}}\right\}
\end{equation*}
\emph{where $q\geq 1$, $C>0$, $s>0$. \\
Then there  exists $K>0$, such that for $|k| > K$ there holds}
\begin{equation*}
 \mbox{if} \quad u \in W, \ |u_k|=\frac{C}{|k|^s q^{|k|}}, \qquad \mbox{then} \qquad  u_k \cdot F_k(u) <0.
\end{equation*}

For the proof of  the above fact see Theorem 3.1 and its proof in \cite{ZKS3}, where the case with $q=1$ was treated.

Projection of the set $W$ onto $k^{\mathrm{th}}$ mode is a closed disc (or interval) centred at zero and of radius
$r_k =\frac{C}{|k|^s q^{|k|}}$. Geometrically the isolation property means that if $|u_k|=r_k$ for some $k> K$ then the $k$-th component of the vector field is pointing inwards the set. As a consequence, the only way a trajectory may leave the set $W$ forward in time is by increasing some of leading modes $|u_k|$, $k\leq K$ above the threshold $r_k$. However, one has to be careful with what "inwards" means in the above statement because $W$ has empty interior as a compact subset in infinite dimensional space.


This property is used   in  our approach to obtain a priori bounds for $u_k(h)$ for small $h>0$ and $|k|>K$, while the leading modes $u_k$ for $|k| \leq K$ are computed using  tools for rigorous integration of ODEs \cite{CAPDREVIEW,Lo,NJP} based on the interval arithmetics \cite{Mo}, i.e. to obtain set $W$ as in Theorem~\ref{thm:limitLN}. Moreover, from the point of view of topological method, the isolation property is of crucial importance as it shows that on the tail we have the entry behaviour, which enable us to apply the finite dimensional tools from the dynamics.


In this work we use sets of the type described above with $s=0$ and $q>1$. The isolation property for KS equation on such sets is established in \cite[Rem. 19]{WZ}.



\subsection{Variational system}

Assume that all assumptions of Theorem \ref{thm:limitLN} are
satisfied. From first assertion   of Theorem
\ref{thm:limitLN} it follows  that
\begin{equation*}
  \varphi^n(t,P_nu) \to \varphi(t,u),
\end{equation*}
and the convergence is uniform on $[0,T] \times Z$.

Now let us consider the variational matrix for $\varphi^n$ given
by
\begin{equation*}
  V^n_{ij}(t,u)= \frac{\partial \varphi^n_i}{\partial u_j} (t,u).
\end{equation*}



To see why we expect the convergence  here for systems with diagonal $L$   let us remark, that
$V^n$ satisfies the following differential equation
\begin{equation*}
  \frac{d V_{ij}^n}{dt}=  \lambda_i V^n_{ij} + \sum_k \frac{\partial  N_i}{\partial u_k} V^n_{kj}
\end{equation*}
with initial condition $V(0)=\mathrm{Id}$.
The above equation has the same strong damping as the original equation (\ref{eq:feqLN}). Observe that the bound
for Lipschitz constant in equation (\ref{eq:LipConstant}) for equation (\ref{eq:feqLN}) and its Galerkin
projections is also a uniform bound for the norms of matrices
$V^n(t)$ for $t\in[0,T]$.  Once we have a strong damping
and a-priori bounds for $V^n$  we can  use logarithmic norms  to
control the convergence of $V^n$'s to variational matrix for (\ref{eq:feqLN}). In \cite{Z1} this has been done under assumption about $W$ being a trapping region. Moreover,
one additional condition was needed - (see  condition \VL formulated in Def.~\ref{def:condV}).


Since each column in $V^{n}_{ij}$ evolves separately, we consider the system of variational equations
\begin{eqnarray}
  \frac{d}{dt} x^n &=& P_nF(x^n), \quad x^n \in H_n,  \label{eq:sysVar1} \\
  \frac{d}{dt} C^n &=& D P_nF_{|H_n}(x^n) C^n, \quad C^n \in H_n. \label{eq:sysVar2}.
\end{eqnarray}
The above system has $H_n \times H_n \subset H \times H$ as the phase-space.

To bring the variational system to the setting discussed in this section we proceeded as follows.
On $H \times H$ we use norm $\|(x,v)\|=\max(\|x\|,\|v\|)$. This makes $H\times H$ a \gss space. The Galerkin projection $P_n$ on $H\times H$ is defined by  $P_n(x,c)=(P_nx,P_nc)$.

In $H \times H$ we can formally write the variational system
\begin{eqnarray}
  \frac{d}{dt} x &=& F(x),  \label{eq:sysVar1-H} \\
  \frac{d}{dt} C &=& DF(x) C, \label{eq:sysVar2-H}
\end{eqnarray}
or
\begin{equation}
  \frac{d}{dt} (x,C)=F_V(x,C).  \label{eq:sysVarH}
\end{equation}
Observe that $\pi_i F_{V}(x,C)$ for $i \in \mathbb{Z_+}$ is a formal power series in variables $x_k$ and $C_k$.





\begin{definition}
\label{def:condV}
Let  $F$ on $W$ satisfies conditions C1,C2,C3,C4,D.
We say that (\ref{eq:sysVar1},\ref{eq:sysVar2}) satisfies condition \VL on $W \times W_c\subset H \times H$, if the following conditions hold  \newline
\begin{itemize}
\item[\VL{}-C1] there exists $M_c \geq 1$, such that $P_n W_c \subset W_c$ for all $n \geq M_c$
\item[\VL{}-C2] $W_c$ is compact.
\item[\VL{}-C3] $W \times W_c \subset \dom(F_V)$, \\
(i.e. for each $(u,C) \in W \times W_c$  sequence $\{\widetilde{DF}_i(u)C\}_{i \in \mathbb{Z}_+}$ belongs to $H$)
and function $F_V:W \times W_c \to H\times H$ given by \\
 $F_V(u,C)=(F(u),\{\widetilde{DF}_i(u)C\}_{i \in \mathbb{Z}_+})$  is continuous,
\item[\VL{}-D] there exists $A \in \mathbb{R}$, such that
for any $n$ holds
\begin{equation*}
  \sup_{(x,v) \in  P_n(W \times W_c)} \mu(D P_n F_{V|H_n \times H_n}(x,v))  \leq A.
\end{equation*}
\end{itemize}
\end{definition}



The following theorem is a generalization  of \cite[Thm. 2]{Z1} is proven in \cite{WZ24} \textbf{PZ: dac lepsze wspolrzedne}
\begin{theorem}
\label{thm:c1conver} Same assumptions as in Theorem
\ref{thm:limitLN}.

Assume that condition  \textbf{C4}  is satisfied on $W$.  Assume that $Z$ is convex.

Assume that we have a family $W_{C_j} \subset H$ of compact and convex sets, such that  condition \VL is satisfied on $W \times W_{C_j}$ and
for any $n >j$ solution of the variational problem (\ref{eq:sysVar1}--\ref{eq:sysVar2}) with initial conditions $x^n(0) \in Z$ and $C^n(0)=e_j$ satisfies
\begin{equation*}
  C^n(t) \in W_{C_j}, \quad t \in [0,T]
\end{equation*}




Then there exists a family of continuous functions
$V_{ij}:[0,T]\times Z \to {\mathbb R}$ for $i,j=1,\dots,\infty$, such that
\begin{description}
\item[convergence:] For each $j$ the function $V^n_{\ast j}(t,P_n z)$
converges to $V_{\ast j}(t,z)$ uniformly on $[0,T] \times Z$,  and
there exists $V(t,x) \in \mbox{Lin}(H,H)$, such that
\begin{eqnarray*}
  \|V(t,x)\| &\leq& e^{l t}, \quad (t,x) \in [0,T] \times Z,\\
   V(t,x)e_j &=& \sum_i V_{ij}(t,x)e_i,
\end{eqnarray*}
and for every $a \in H$ the map $[0,T] \times Z \ni (t,x) \mapsto V(t,x)a$ is continuous.


\item[smoothness:]  For any $x,y \in Z$ and any $t\in[0,T]$ we have
\begin{equation}
  \varphi(t,x) - \varphi(t,y) =  \int^1_0 V(t,y+s(x-y))ds \cdot (x - y),
    \label{eq:intpar}
\end{equation}
and  for every $j$ partial derivative of the flow $\frac{\partial \varphi}{\partial u_j}(t,u)$ exists and
\begin{equation}
  \frac{\partial \varphi}{\partial u_j}(t,u)=V_{\ast j}(t,u).  \label{eq:dfiduj=Vij}
\end{equation}
\item[equation for $V$:]  $V(t,u)$ satisfies the following variational equation
  \begin{equation}
     \frac{d V_{*j}}{dt}(t,u) = \sum_i e_i \sum_k \frac{\partial F_i}{\partial u_k}(\varphi(t,u))
           V_{kj}(t,u), \label{eq:varinfdim}
  \end{equation}
 with the initial condition $V(0)=\mathrm{Id}$ in the following sense:  for each $j$ the derivative  $\frac{d V_{j}}{dt}(t,u)$ exists, the series on r.h.s. of (\ref{eq:varinfdim}) converges uniformly
 on $[0,T] \times Z$ and equation (\ref{eq:varinfdim}) is
 satisfied.
\end{description}
\end{theorem}







==> ks_convergence_cond.tex <==
\section{Convergence conditions for the KS equation}
\label{sec:ConvergenceCondKs}

The following lemma has been proven in \cite{WZ24}.
\begin{lemma}{\cite[Lemma 2]{WZ24}}
\label{lem:compt-gss}
  Assume that $H$ is \gss. Then $W \subset H$ is compact, iff it is closed, bounded and we have \textbf{uniform bound on the tail}, i.e. for every $\epsilon >0$ there exists $N$, such that
  for all $n \geq N$ for all $w \in W$ holds $\|(I-P_n)w\| < \epsilon$.
\end{lemma}


In what follows we assume that $H=c_0$ is a space of sequences converging to zero with norm supremum norm $\|u\|=\sup_{n} |u_n|$.





For $S >0$ and $q>1$ we define
\begin{equation*}
  \WqS{q}{S}=\left\{(u_k)_{k=1}^\infty\in H : |u_k|\leq Sq^{-k}\right\}.
\end{equation*}


From  (\ref{eq:fuKS}) we see that
\begin{eqnarray}  \label{eq:partialDerKS}
  \frac{\partial F_i}{\partial z_k}(z)=   \left\{
                                         \begin{array}{ll}
                                           2i \omega(i,k) z_{|i-k|} + 2i z_{i+k}, & \hbox{ for $k \neq i$;} \\
                                           i^2(1-\nu i^2) +  2i z_{i+k}, & \hbox{for $i=k$;} \\
                                         \end{array}
                                       \right.,
\end{eqnarray}
where $\omega(i,k)=-1$ if $i>k$ and $\omega(i,k)=1$ if $i<k$.

\begin{lemma}
\label{lem:DerKS-bnds}
  For $z \in \WqS{q}{S}$ holds
\begin{eqnarray}  \label{eq:DerKS-bnds}
    \left|\frac{\partial F_i}{\partial z_k}(z)\right| \leq  \left\{
                                         \begin{array}{ll}
                                           4i S q^{-|i-k|}, & \hbox{ for $k \neq i$;} \\
                                           |i^2(1-\nu i^2)| +  2i S q^{-(i+k)}, & \hbox{for $i=k$;} \\
                                         \end{array}
                                       \right.
\end{eqnarray}
\end{lemma}



\begin{theorem}
\label{thm:conv-cond-KS}
Let $W=\WqS{q}{S}$ for some $S\geq 0$, $q>1$. Then the conditions \textbf{C} for the KS equation (\ref{eq:fuKS}) is satisfied on $W$.
\end{theorem}
\textbf{Proof:}

\noindent\textbf{C1:} We have to show that $F|_W$ is continuous. For $u\in \WqS{q}{S}$ we have (see (\ref{eq:fuKS}))
	\begin{multline}\label{eq:KSFbound}
		|F_k(u)| \leq S q^{-k}|k^2(1-\nu k^2)| + k\sum_{n=1}^{k-1}Sq^{-n}Sq^{n-k} + 2k\sum_{n=1}^\infty Sq^{-n}Sq^{-n-k} \\ = S q^{-k}|k^2(1-\nu k^2)| + k(k-1)S^2q^{-k} + 2kS^2q^{-k}(q^2-1)^{-1} \\
		\leq Sq^{-k}\left(\nu k^4 + k^2 + Sk(k-1)+2k^2S(q^2-1)^{-1}\right) \leq C k^4 q^{-k},
	\end{multline}
for some $C=C(S,q)$. Hence $\lim_{k_\to\infty}|F_k(u)| = 0$ and thus $F(u)\in H$.

Observe that from the above computations follows that $F_k : W \to \mathbb{R}$ is continuous as a limit of uniformly convergent functions $F_k P_n$, which are continuous on $W$.

	
	We will prove that $F$ is (uniformly) continuous on $W$. Let us fix $\varepsilon>0$. For any $u,v\in W$ using uniform bound (\ref{eq:KSFbound}) we obtain
	$$|F_k(u)-F_k(v)|\leq |F_k(u)| +|F_k(v)|\leq 2Ck^4q^{-k}.$$
 Hence, there exists $M\in\mathbb N$ such that for $k>M$ and for all $n\in\mathbb Z_+$ there holds
\begin{equation*}
\|(I-P_M)F(u)-(I-P_M)F(v)\|\leq \varepsilon,  \quad \forall u,v \in W.
\end{equation*}

From continuity of $F_k$ it follows that $P_M F$ is uniformly continuous on $W$, hence there exists $\delta >0$ such that
\begin{equation*}
  \|P_M F(u) - P_M F(v)\| \leq \varepsilon, \quad \mbox{if $\|u-v\| \leq \delta$}.
\end{equation*}
Thus $F$ is continuous on $W$.\\

\noindent\textbf{C2:} We have to show that there is $l\in\mathbb R$ such that for all $n\in\mathbb Z_+$ there holds $\sup_{x\in P_nW} \mu\left(DF^n(x)\right)\leq l$. 

Let $n$ be dimension of the Galerkin
projection. Formula (\ref{eq:logNormMax}) implies that
\begin{equation*}
  \mu\left(D P_n F_{|H_n}(z) \right)=\max_{i\leq n} R_{i,n}(z),
\end{equation*}
where for any $i \leq n$  $R_{i,n}(z)$  is defined and estimated using  Lemma~\ref{lem:DerKS-bnds}  for $z \in P_n W$ as follows
\begin{multline}\label{eq:RiInfty}
R_{i,n}(z):=\frac{\partial F_i}{\partial z_i}(z) +  \sum_{k\neq i, k=1}^n \left| \frac{\partial F_i}{\partial z_k}(z) \right| \\
\leq i^2(1-\nu i^2) + 2i Sq^{-2i} + \sum_{k, k \neq i}4i S q^{-|i-k|} \\
 \leq i^2(1-\nu i^2) +  2i Sq^{-2i} + 8i S \sum_{k=1}^\infty q^{-k} \\   
 \leq  i^2(1-\nu i^2)  + 8iS (\frac{1}{q-1} +  q^{-2i})=: R_{i,\infty}.
\end{multline}
We see that $R_{i,\infty} \to -\infty$ if $i \to \infty$.  It is immediate that there exists $l \in \mathbb{R}$ for all $z \in P_nW$ holds
\begin{eqnarray*}
\mu\left(D P_n F_{|H_n}(z) \right)=\max_{i\leq n} R_{i,n}(z) \leq \sup_{i} R_{i,\infty}  =l.
\end{eqnarray*}
\qed


\begin{lemma}\label{lem:KSVconv}
Let us fix $z\in W=\WqS{q}{S}$ and define a sequence $V_k=\frac{\partial F_i}{\partial z_k}(z)$. Then $Vu = \sum_{k}V_ku_k$ defines a functional $V\in H^*$ and 
$$V=\lim_{n\to\infty} D(F_i|_{H_n})(P_nz) = \widetilde{DF_i}(z)$$
with the norm $\|V\|\leq K i^4$, for some $K \geq 0$. Moreover, $\widetilde{DF_i}(z)$ is continuous on $W$.
\end{lemma}
\textbf{Proof:}
First we will show that $V\in H^*$. For $z\in W$ and $u\in H$ formula (\ref{eq:DerKS-bnds}) gives
\begin{multline*}
	\sum_{k=1}^\infty|V_ku_k|\leq \|u\|\sum_{k=1}^\infty\left|\frac{\partial F_i}{\partial z_k} \right| \leq \|u\|\left(|i^2(1-\nu i^2)| + 2iS q^{-2i} + 8iS\sum_{k=1}^\infty q^{-k}\right) \\
	= \|u\|\left(|i^2(1-\nu i^2)| + 2i Sq^{-2i} + 8iS(q-1)^{-1}\right).
\end{multline*}
Hence $V\in H^*$ and $\|V\|\leq Ki^4$ for some $K>0$.

Now we will show that $\widetilde{DF_i}(z)=V$. It is easy to see that for $n \geq i$ holds
\begin{equation*}
	\left(V-D(F_i|_{H_n})(P_nz)\right)u= 2i \left(\sum_{k>n} z_{k-i} u_k + \sum_{k>n-i} z_{i+k}u_k\right)
\end{equation*}

Therefore for $u\in H$, $\|u\|=1$ we have
\begin{multline*}
	\left|\left(V-D(F_i|_{H_n})(P_nz)\right)u\right| \leq  2i \sum_{k>n} |z_{k-i}| +  2i \sum_{k>n-i}^\infty|z_{i+k}| \\
	\leq  4iS\sum_{k=n-i+1}^\infty q^{-k} = 4iSq^{i-n}(q-1)^{-1}.	
\end{multline*}
Hence $\lim_{n\to\infty}\left\|\left(V-D(F_i|_{H_n})(P_nz)\right)\right\|=0$.

There remains to show that $\widetilde{DF_i}$ is continuous on $W$. Let us fix $\varepsilon >0$. Let us denote $V(z)=\widetilde{DF_i}(z)$ for $z \in W$.  Then for $u\in H$ such that $\|u\|=1$ we have
\begin{eqnarray*}
	\|(V(v)-V(z))u\| \leq \sum_{k=1, k\neq i}^\infty 2i|z_{|i-k|}-v_{|i-k|}| + 2i\sum_{k=1}^\infty|z_{i+k}-v_{i+k}|\\
	\leq 6i\sum_{k=1}^\infty|z_k-v_k|.
\end{eqnarray*}
There is $M\in\mathbb N$ such that  for all  $z,v\in W$   there holds $\sum_{k=M+1}^\infty|z_k-v_k|\leq \varepsilon/2$. Now if $\|v - z\| \leq  \delta$, then $\sum_{k=1}^M|z_k-v_k|\leq M \delta \leq \varepsilon/2$ for $\delta$ small enough. Summarizing, for sufficiently small $\delta$  there holds
\begin{equation*}
	\|V(v)-V(z)\| \leq 6i\varepsilon, \quad \mbox{if $\|z-v\| \leq \delta$, $z,v \in W$}
\end{equation*}
and thus $\widetilde{DF_i}$ is continuous on $W$.\qed


\begin{theorem}
\label{thm:Vl-cond-KS}
Let $W=\WqS{q}{S}$ and $W_c=\WqS{q}{S_c}$ for some $q>1$ and $S,S_c\geq 0$. Then the system (\ref{eq:c0IVP})-(\ref{eq:c1IVP}) for the KS equation (\ref{eq:fuKS}) satisfies condition \VL on $W\times W_c$.
\end{theorem}	
\textbf{Proof:}

\noindent\textbf{VC1}: Recall that $H$ is a space of sequences converging to zero with supremum norm. Let us fix $(u,C)\in W\times W_c$. Firstwe will show that $F_V$ is well defined, that is $\{\widetilde{DF_i}(u)C\}_{i \in \mathbb{Z_+}} \in H$. We have to show that $\lim_{i\to \infty} \widetilde{DF_i}(u)C=0$. From (\ref{eq:DerKS-bnds}) and using $|u_{k}|\leq Sq^{-k}$ and $|C_k|\leq S_cq^{-k}$ we obtain
\begin{equation}\label{eq:uniformBoundOnDfuC}
	\begin{array}{rcl}
	|\widetilde{DF_i}(u)C| &\leq& |i^2(1-\nu i^2)C_i| + 2 i  Sq^{-2i} |C_i| + 4i S \sum_{k,k \neq i} q^{-|i-k|} |C_k|\\
	&\leq& |i^2(1-\nu i^2)| S_c q^{-i}  + 2i S S_c q^{-3i} + 4i S S_c \sum_{k,k \neq i} q^{-|i-k| - k} \\
	&\leq& S_cq^{-i}\left(|i^2(1-\nu i^2)|  + 2i S q^{-2i} + 4i^2 S + 4i S \sum_{k >i } q^{2i-2k}\right) \\
	&\leq& S_cq^{-i}\left(|i^2(1-\nu i^2)|  + 2i S q^{-2i} + 4i^2 S + 4i S \frac{1}{q^2 -1}\right)\\
	&\leq& K_1i^4q^{-i}
	\end{array}
\end{equation}
for some $K_1\geq 0$. Hence $\lim_{i\to \infty} \widetilde{DF_i}(u)C=0$ and thus $\{\widetilde{DF_i}(u)C\}_{i\in\mathbb Z_+}\in H$.

Now we will show that $F_V(u,C)=(F(u),\{\widetilde{DF_i}(u)C\}_{i\in\mathbb Z_+})$ is continuous on $W\times W_c$. From \textbf{C1} we know that $F(u)$ is continuous, so there remains to check continuity of the second component.  Recall, we are working with supremum norm and thus what we have to show is that 
$$
\sup_{i\in\mathbb Z_+}|\{\widetilde{DF_i}(u)C_u\}_{i\in\mathbb Z_+}-\{\widetilde{DF_i}(v)C_v\}_{i\in\mathbb Z_+}|< \varepsilon
$$
if $\|C_u-C_v\|$ and $\|u-v\|$ are small enough.  

Let us fix $\varepsilon>0$. From (\ref{eq:uniformBoundOnDfuC}) there is $M>0$ such that for all $i>M$ and  $(u,C)\in W\times W_c$ there holds
\begin{equation*}
	|\widetilde{DF_i}(u)C | < \varepsilon/2.  
\end{equation*}	
Thus for $i>M$, $u,v\in W$ and $C_u,C_v\in W_c$ we have 
\begin{equation}\label{eq:tailDFiC}
|\{\widetilde{DF_i}(u)C_u\}_{i\in\mathbb Z_+}-\{\widetilde{DF_i}(v)C_v\}_{i\in\mathbb Z_+}|< \varepsilon.
\end{equation}
Let us fix this $M$ and now we will consider indices $i\leq M$. 

From Lemma~\ref{lem:KSVconv} the functions $\widetilde{DF_i}$ are continuous on the compact set $W$ and thus bounded. There is a constant $K_2$ such that
\begin{equation}
\|\widetilde{DF_i}(u)\|\leq K_2, \quad u\in W, i\leq M.  \label{eq:DFinorm}
\end{equation}
Again from uniform continuity of  $\widetilde{DF_i}$ on $W$ it follows that there exists $\delta>0$, such that for all $u,v \in W$ such that
\begin{equation}
 \|\widetilde{DF_i}(u) - \widetilde{DF_i}(v)\| < \frac{\varepsilon}{2S_c}, \quad i=1,\dots,M , \qquad \mbox{if $\|u-v\| \leq \delta$}.   \label{eq:DFidiff}
\end{equation}

Now, for $(u,C_u),(v,C_v) \in W \times W_c$, such that $\|u - v\| \leq \delta$ and $\|C_u-C_v\|\leq \frac{\varepsilon}{2K_2}$ and $i \leq M$ we obtain (we use (\ref{eq:DFinorm}) and (\ref{eq:DFidiff}))
\begin{multline*}
	|\widetilde{DF_i}(u)C_u-\widetilde{DF_i}(v)C_v| \leq |\widetilde{DF_i}(u)(C_u-C_v)|+|(\widetilde{DF_i}(u)-\widetilde{DF_i}(v))C_v|\\
	\leq \|\widetilde{DF_i}(u)\|\cdot \|C_u-C_v\|+ \|\widetilde{DF_i}(u)-\widetilde{DF_i}(v)\|\cdot \|C_v\| \\
	< K_2 \cdot \|C_u-C_v\| +\max_{C \in W_c}\|C\| \frac{\varepsilon}{2S_c} < \varepsilon.
\end{multline*}	
Summarizing, from (\ref{eq:tailDFiC}) and the above estimate we obtain
$$
 \sup_{i\in\mathbb Z_+}|\{\widetilde{DF_i}(u)C_u\}_{i\in\mathbb Z_+}-\{\widetilde{DF_i}(v)C_v\}_{i\in\mathbb Z_+}|< \varepsilon
$$
if $\|u - v\| \leq \delta$ and $\|C_u-C_v\|\leq \frac{\varepsilon}{2K_2}$. Thus $F_V$ is continuous.
\vskip\baselineskip
\noindent\textbf{VC2:} We have to find a uniform bound on logarithmic norms of 
 $DP_nF_V|_{H_n\times H_n}$, for $n\in\mathbb Z_+$. Such derivative is of the following form
\begin{eqnarray*}
M^n:=DP_nF_V|_{H_n\times H_n}(u,C) \\
= \begin{bmatrix}
	DP_nF|_{H_n}(P_nu) & 0 \\
	\left\{D(\widetilde{DF_i}|_{H_n}(P_nu))P_nC\right\}_{i\leq n} & DP_nF|_{H_n}(P_nu)
\end{bmatrix}.
\end{eqnarray*}
Let us denote blocks of the above matrix by $M^n=\begin{bmatrix}A^n & 0 \\ B^n & A^n\end{bmatrix}$. Recall, that the logarithmic norm related to the supremum norm (see (\ref{eq:logNormMax})) is given by $\mu(M^n) =\max_{i} M^n_{ii} + \sum_{k\neq i}|M^n_{ik}|$.  It is immediate that this maximum is realized for rows related to variables $C_i$.

From  (\ref{eq:partialDerKS}) it follows that $C_i$-th component of $F_V$ denoted by $F_{V,C_i}$ is given by
\begin{equation*}
  F_{V,C_i}=2i \sum_{j,j\neq i} \omega(i,j) z_{|i-j|}C_j + 2i \sum_{j} z_{i+j}C_j + i^2(1-\nu i^2)C_i,
\end{equation*}
hence
\begin{equation*}
  \frac{\partial F_{V,C_i}}{\partial z_k}(z,C)=\left\{
                                                \begin{array}{ll}
                                                  -2i C_{i-k} + 2i C_{i+k}, & \hbox{$i >k$;} \\
                                                  2i C_{i+k} + 2i C_{k-i}, & \hbox{$i<k$;} \\
                                                  2i C_{2i}, & \hbox{$i=k$.}
                                                \end{array}
                                              \right.
\end{equation*}
The sum related to  $C_i$-th row for $n$-th Galerkin projection has the following form (see (\ref{eq:RiInfty}) for the definition of $R_{i,n}(z)$ and $R_{i,\infty}$)
\begin{eqnarray*}
 R_{C_i,n}(z,C):=\sum_{k=1}^n \left|\frac{\partial P_n F_{V,C_i}}{\partial z_k}(P_n z,P_n C) \right| + R_{i,n}(z) \\
\leq 2i \sum_{k=1, k \neq i}^\infty |C_{|i-k|}| + 2i \sum_{k=1}^\infty |C_{i+k}| + R_{i,\infty}
\leq 6i \sum_{k=1}^\infty |C_{k}| + R_{i,\infty} \\
= 6i S_c \frac{1}{q-1} + i^2(1-\nu i^2)  + i S (\frac{1}{q-1} +  q^{-2i})=: R_{C_i,\infty}
\end{eqnarray*}
We see that $R_{C_i,\infty} \to -\infty$ if $i \to \infty$.  It is immediate that there exists $L \in \mathbb{R}$
\begin{eqnarray*}
 R_{C_i,\infty} \leq L.
\end{eqnarray*}
This finishes the proof of condition \textbf{VC2}.
\qed


==> lineqestm.tex <==

\section{Estimates for non-au\-to\-no\-mous linear \\ equa\-tions}
\label{sec:estmlinEq}

Theorem~\ref{thm:limitLN} guarantees that within sets satisfying the \emph{convergence conditions} the objects we are going to compute (or estimate) indeed exists. The rough estimates from this theorem, in particular bound on the Lipschitz constant $\|V(t,x)\|\leq e^{lt}$, are of minor practical relevance. To make our algorithm work efficiently we need more subtle tools, which give us more accurate bounds for particular coordinates or blocks of coordinates. The goal of this section is to present tools, which will allow us estimate norms of blocks of the variational matrix $V(t,x)$.

\subsection{Block decomposition of a non-autonomouos linear ODE}
The content of this subsection is based on the results from \cite{KZ}. 
\begin{definition}
	%\label{def:solOde}
	Let $f :U \to \mathbb{R}^n$, where  $U \subset \mathbb{R}^n$ is open and let $D \subset \mathbb{R} $ be an interval.
	An absolutely continuous function $x:D \to \mathbb{R}^n$ is a \emph{weak solution} of
	\begin{equation*}
		x'=f(x),\ x(t_0)=x_0,\quad  t_0\in D,\ x\in \mathbb{R}^n.% \label{eq:wode}
	\end{equation*}
	if for all $t \in D$ there holds
	\begin{equation*}
		x(t) = x_0 + \int_{t_0}^t f(x(s)) ds.%  \label{eq:inteq}
	\end{equation*}
\end{definition}

The next lemma follows immediately from \cite[Lemma 4.1]{KZ}.
\begin{lemma}
 \label{lem:comp-lin-problems}
   Assume that $W:[0,T] \to {\mathbb
R}^{k\times k}$ is an absolutely continuous
map, which is a weak solution of the equation
\begin{equation*}
  W'(t)=A(t) \cdot W(t),
\end{equation*}
where  $A:[0,T]\to {\mathbb R}^{k \times k}$ is bounded and measurable. Assume that we have a decomposition $\mathbb R^{k}=\bigoplus_{i=1}^n \mathbb{R}^{k_i}$ and denote by $A_{ij}\in
\mathrm{Lin}(\mathbb{R}^{k_i},\mathbb{R}^{k_j})$, $i,j=1,\ldots,n$ the blocks $A$ corresponding to this decomposition, that is for $z=(z_1,\ldots,z_n)\in\bigoplus_{i=1}^n\mathbb{R}^{k_i}$ we have 
$$	Az= \sum_{j=1}^n A_{ij}z_j.$$

Let $J:[0,T] \to \mathbb{R}^{n \times n}$ be a measurable matrix function satisfying the following inequalities for all $t \in [0,T]$
\begin{equation*}
%\label{eq:def-JL2}
J_{ij}(t) \geq
  \begin{cases}
      \|A_{ij}(t) \|  & \text{for $i \neq j$}, \\
     \mu(A_{ii}(t))  & \text{for $i=j$}.
  \end{cases}
\end{equation*}

If $B:[0,T] \to \mathbb{R}^{n \times n}$ is a weak solution of the
problem
\begin{equation*}
   B'(t)=J(t)B(t)
\end{equation*}
with initial conditions satisfying
\begin{equation*}
  B_{ij}(0) \geq \|W_{ij}(0)\|, \quad i,j=1,\dots,n
\end{equation*}
then
\begin{equation*}
  \|W_{ij}(t)\| \leq B_{ij}(t), \quad t \in [0,T],  \quad i,j=1,\dots,n.
\end{equation*}
\end{lemma}


\subsection{Block decomposition of variational equation}
%\label{subsec:blockdecmp}
We would like to adapt Lemma~\ref{lem:comp-lin-problems} to the variational equation for dissipative PDEs and its solution obtained as the limit of solutions of variational equation as in Theorem~\ref{thm:limitLN}. We will consider a very particular decomposition
\begin{equation*}
 H=\bigoplus_{k \leq m} \langle e_k \rangle   \oplus Y, \quad Y=(I-P_m)H
 \end{equation*}
with $m$ 1-dimensional subspaces $\langle e_i \rangle$ and infinite-dimensional subspace $Y$.

To  distinguish between $V_{ij}$, when $i,j$ are treated as indices of particular coordinates and the situation when they are supposed to denote blocks (as in Lemma~\ref{lem:comp-lin-problems}) for the block entries involving $Y$ we will write $V_{yy}$, $V_{iy}$, $V_{yi}$. In this way $V_{ij}$ for any $i,j$ will denote always a number in the matrix $V$.


 The block notation introduced above make sense also for $F^n$ (the vector field for Galerkin projection). Below we write $\frac{\partial F^n}{\partial y}$
meaning that the partial derivatives are meant with respect $y \in P_n y$, i.e. this is finite dimensional matrix.


The following theorem has been proven in \cite{WZ24}.
\begin{theorem}{\cite[Theorem 15]{WZ24}}
\label{thm:lineqestm-inf}
Same assumptions and notation as in Theorem~\ref{thm:limitLN}. For some $m>0$ let us consider the following decomposition of $H$
 \begin{equation*}
 H=\bigoplus_{k \leq m}  \langle e_k  \rangle    \oplus Y, \quad Y=(I-P_m)H.
 \end{equation*}



 Assume that matrix $J \in \mathbb{R}^{(m+1) \times (m+1)}$ satisfies
\begin{equation*}%\label{eq:def-J}
 J_{ij} \geq
  \begin{cases}
     \sup_{n>m} \sup_{w \in W} \left\|\frac{\partial F^n_i}{\partial u_j}(w) \right\|,  & \text{for $i \neq j$, $i,j \leq m$}, \\
      \sup_{n>m} \sup_{w \in W}  \frac{\partial F^n_i}{\partial u_j}(w),   & \text{for $i=j$, $i\leq m$}, \\
     \sup_{n>m} \sup_{w \in W}  \mu\left(\frac{ \partial F^n_y }{\partial y}(w) \right),     & \text{for $i=j=m+1$} \\
     \sup_{n>m}   \sup_{w \in W} \left\|\frac{ \partial F^n_i}{\partial y}(w) \right\|,  & \text{for $i \leq m$, $j=m+1$} \\
       \sup_{n>m}  \sup_{w \in W} \left\| \frac{\partial  F^n_y}{\partial u_j}(w) \right\|,  & \text{for $i=m+1$, $j \leq m$}.
  \end{cases}
\end{equation*}


Then for any  $u \in Z$ and  $t \in [0,h]$
holds
\begin{eqnarray*}
  |V_{ij}(t,u)| &\leq&  \left(e^{Jt}\right)_{ij},  \quad i,j=1,\dots,m,  \\% \label{eq:Vij-estm}\\
  \|V_{yj}(t,u)\|  &\leq&  \left(e^{Jt}\right)_{m+1,j},  \quad j=1,\dots,m,\\%  \label{eq:Vyj-estm} \\
  \|V_{iy}(t,u) \| &\leq&  \left(e^{Jt}\right)_{i,m+1}, \quad i=1,\dots,m, \\% \label{eq:Vjy-estm} \\
  \|V_{yy}(t,u)\| &\leq&  \left(e^{Jt}\right)_{m+1,m+1}. % \label{eq:Vyy-estm}
\end{eqnarray*}
\end{theorem}




==> lognorm.tex <==
\section{Logarithmic norms}
\label{sec:lognorm}


\textbf{PZ: jest tez w \cite{WZ24} - nie wiem czy czegos nie skrocic - wyrzucic}

\begin{definition} \cite{D58,L58}
\label{def:lognorm}
 Let $\| \cdot \|$ denote a vector norm on $\mathbb{R}^n$  as
well as its subordinate operator norm on $\mathbb{R}^{n
\times n}$. The \emph{logarithmic
norm} of operator $A$ is
\begin{equation*}
  \mu(A)=\lim_{h \to 0^+} \frac{\|\mathrm{Id} + hA \| - 1}{h}
\end{equation*}
\end{definition}
For the properties and the use of the logarithmic norm see \cite{KZ} and the literature given there.



Consider the differential equation
\begin{equation}
  x'=f(x), \quad \mbox{$f \in C^1$}. \label{eq:odelogn}
\end{equation}
Let $\varphi(t,x_0)$  denote the solution of equation
(\ref{eq:odelogn}) with the initial condition $x(0)=x_0$. By $\|x
\|$ we denote a fixed arbitrary norm in $\mathbb{R}^n$.


From Lemma~\ref{lem:boundOnVariationalLinEq} one can easily derive the following result.
\begin{lemma}
\label{lem:estmLogN} Let $y:[0,T] \to \mathbb{R}^n$ be a piecewise
$C^1$ function and $\varphi(\cdot,x_0)$ be defined for $t \in
[0,T]$. Suppose that $Z$ is a convex set such that   the following
estimates hold:
\begin{eqnarray*}
  y([0,T]), \varphi([0,T], x_0) \in Z  \\
  \mu\left(\frac{\partial f}{\partial x}(\eta)\right) \leq l,\quad \mbox{ for $\eta \in Z$} \\
  \left\| \frac{dy}{dt}(t) - f(y(t)) \right\| \leq \delta.
\end{eqnarray*}
Then for $0 \leq t \leq T$ there is
\begin{displaymath}
 \| \varphi(t,x_0) - y(t)  \| \leq e^{lt}  \|y(0) - x_0 \| + \delta \frac{e^{lt} -1}{l},\quad \mbox{if $l \neq 0$}.
\end{displaymath}
For $l=0$, there is
\begin{displaymath}
 \| \varphi(t,x_0) - y(t)  \| \leq  \|y(0) - x_0 \| + \delta t.
\end{displaymath}
\end{lemma}


In the paper we frequently use norm  $\|x\|_{\infty}=\max_{i=1,\dots,n} |x_i|$ on $\mathbb{R}^n$.
\begin{lemma}
\label{lem:logNormMax}
  Let $A \in \mathbb{R}^{n \times  n}$, then the logarithmic norm of $A$ induced by norm $\| \cdot \|_\infty$ is given by
  \begin{equation}
    \mu(A)=\max_{i=1,\dots,n} \left( A_{ii} + \sum_{k=1 , k\neq i}^n |A_{ik}| \right). \label{eq:logNormMax}
  \end{equation}
 \end{lemma}

